Precision Measurement of the B to X_s \gamma Photon Energy Spectrum, Branching Fraction, and Direct CP Asymmetry A_{CP}(B to X_{s+d}\gamma

The photon spectrum in the inclusive electromagnetic radiative decays of the $B$ meson, $B \to X_{s} \gamma$ plus $B \to X_{d} \gamma$, is studied using a data sample of $(382.8 \pm 4.2) \times 10^6$ $\Upsilon(4S) \to B\overli\ ne{B}$ decays collected by the \babar\ experiment at SLAC. The spectrum is used to extract the branching fraction ${\cal B}(B \to X_{s} \gamma)=(3.21 \pm 0.33)\times 10^{-4}$ for $E_{\gamma}>1.8 \gev$ and the direct CP asymmetry $A_{CP}(B \to X_{s+d} \gamma)=0.057 \pm 0.063$. The effects of detector resolution and Doppler smearing are unfolded to measure the photon energy spectrum in the $B$ meson rest frame.

==> abstract.tex <==
The photon spectrum in the inclusive electromagnetic radiative decays of the $B$ meson, $B \to X_{s} \gamma$ 
plus $B \to X_{d} \gamma$, is studied  using a data sample  of $(382.8 \pm 4.2) \times 10^6$ $\Upsilon(4S) \to B\overline{B}$  decays collected by the \babar\ experiment at SLAC. The spectrum is used to extract the  branching fraction 
${\cal B}(B \to X_{s} \gamma)=(3.21 \pm 0.33)\times 10^{-4}$ for $E_{\gamma}>1.8 \gev$ and the direct $CP$ asymmetry 
$A_{CP}(B \to X_{s+d} \gamma)=0.057 \pm 0.063$. The effects of detector resolution and Doppler smearing are unfolded to measure the photon energy spectrum in the $B$ meson rest frame. 


==> description.tex <==
\\
Title:
Precision Measurement of the $ B \to X_{s} \gamma$ Photon Energy Spectrum, 
Branching Fraction, and Direct $CP$ Asymmetry  $A_{CP}(B \to X_{s+d}\gamma$
Authors: The BABAR Collaboration, J.P. Lees  et al.
Comments: 8 pages, 2 postscript figures, submitted to Physical Review Letters
Report-no: BABAR-PUB-12/016, SLAC-PUB-15180
\\
The photon spectrum in the inclusive electromagnetic radiative decays of the $B$ meson, $B \to X_{s} \gamma$ 
plus $B \to X_{d} \gamma$, is studied  using a data sample  of $(382.8 \pm 4.2) \times 10^6$ $\Upsilon(4S) \to B\overline{B}$  decays collected by the \babar\ experiment at SLAC. The spectrum is used to extract the  branching fraction 
${\cal B}(B \to X_{s} \gamma)=(3.21 \pm 0.33)\times 10^{-4}$ for $E_{\gamma}>1.8 \gev$ and the direct $CP$ asymmetry 
$A_{CP}(B \to X_{s+d} \gamma)=0.057 \pm 0.063$. The effects of detector resolution and Doppler smearing are unfolded to measure the photon energy spectrum in the $B$ meson rest frame. 
\\


==> results.tex <==
\begin{table*}[hbt]
\hspace*{1.0cm}
 \begin{center}
\caption{The measured partial branching fraction, first and second moment ($\pm stat. \pm syst. \pm model$) for different ranges of $\eg$ in the B rest frame. }
  \begin{tabular}{|c|c|c|c|c|} \hline
   $\eg~(\mathrm{GeV})$      & $\Delta\BR(\bxsg)~(10^{-4})$                &   $\efmbrest~(\mathrm{GeV})$                             &  $\varbrest~(\mathrm{GeV}^{2})$        \\ \hline
   1.9 to 2.7   & $3.67 \pm 0.29 \pm 0.34 \pm 0.29$    &  $2.288 \pm 0.025 \pm 0.017 \pm 0.015$   &  $0.0328 \pm 0.0040 \pm 0.0023 \pm 0.0036$   \\       
   2.0 to 2.7   & $3.41 \pm 0.27 \pm 0.29 \pm 0.23$    &  $2.316 \pm 0.016 \pm 0.010 \pm 0.013$   &  $0.0266 \pm 0.0026 \pm 0.0010 \pm 0.0020$   \\       
   2.1 to 2.7   & $2.97 \pm 0.24 \pm 0.25 \pm 0.17$    &  $2.355 \pm 0.014 \pm 0.007 \pm 0.011$   &  $0.0191 \pm 0.0019 \pm 0.0006 \pm 0.0015$   \\       
   2.2 to 2.7   & $2.42 \pm 0.21 \pm 0.20 \pm 0.13$    &  $2.407 \pm 0.012 \pm 0.005 \pm 0.008$   &  $0.0116 \pm 0.0014 \pm 0.0004 \pm 0.0005$   \\ \hline
  \end{tabular}
 \end{center}
 \vspace{-0.1in}
\end{table*}

